ClickVOS: Click Video Object Segmentation

Video Object Segmentation (VOS) task aims to segment objects in videos. However, previous settings either require time-consuming manual masks of target objects at the first frame during inference or lack the flexibility to specify arbitrary objects of interest. To address these limitations, we propose the setting named Click Video Object Segmentation (ClickVOS) which segments objects of interest across the whole video according to a single click per object in the first frame. And we provide the extended datasets DAVIS-P and YouTubeVOSP that with point annotations to support this task. ClickVOS is of significant practical applications and research implications due to its only 1-2 seconds interaction time for indicating an object, comparing annotating the mask of an object needs several minutes. However, ClickVOS also presents increased challenges. To address this task, we propose an end-to-end baseline approach named called Attention Before Segmentation (ABS), motivated by the attention process of humans. ABS utilizes the given point in the first frame to perceive the target object through a concise yet effective segmentation attention. Although the initial object mask is possibly inaccurate, in our ABS, as the video goes on, the initially imprecise object mask can self-heal instead of deteriorating due to error accumulation, which is attributed to our designed improvement memory that continuously records stable global object memory and updates detailed dense memory. In addition, we conduct various baseline explorations utilizing off-the-shelf algorithms from related fields, which could provide insights for the further exploration of ClickVOS. The experimental results demonstrate the superiority of the proposed ABS approach. Extended datasets and codes will be available at https://github.com/PinxueGuo/ClickVOS.

==> sections/bio.tex <==
% \section{Biography Section}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig1}}]{Michael Shell}
% Use $\backslash${\tt{begin\{IEEEbiography\}}} and then for the 1st argument use $\backslash${\tt{includegraphics}} to declare and link the author photo.
% Use the author name as the 3rd argument followed by the biography text.
% \end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{TCSVT-ClickVOS/bio/PinxueGuo.jpeg}}]{Pinxue Guo}
received the B.S. degree in intelligence science and technology from Shanghai University in 2021. He is currently pursuing the Ph.D. degree with the Academy for Engineering and Technology, Fudan University, Shanghai, China. His research interests include video object segmentation, video understanding, and computer vision.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{TCSVT-ClickVOS/bio/LingyiHong.jpg}}]{Lingyi Hong}
is currently pursuing the Ph.D degree with the School of Computer Science, Fudan University, Shanghai, China. He received his B.S. degree from Fudan University in 2022. His research interests include computer vision, video understanding, multimodal learning, and 3D vision.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{TCSVT-ClickVOS/bio/XinyuZhou.jpg}}]{Xinyu Zhou}
received the M.Eng. degree from Xiangtan University in 2020. He is currently pursuing Eng.D. degree with the School of Computer Science, Fudan University, Shanghai. His research interests include computer vision, visual object tracking, and semantic segmentation, medical image processing.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{TCSVT-ClickVOS/bio/ShuyongGao.jpg}}]{Shuyong Gao}
received the Ph.D. degree in computer science from Fudan University, Shanghai, China, in 2023. He is currently a Postdoctoral Researcher with Fudan University, Shanghai, China. His research interests include robotics, computer vision, generative models, and salient/camouflage object detection.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{TCSVT-ClickVOS/bio/WanyunLi.jpg}}]{Wanyun Li}
received the B.S. degree in Computer Science and Technology from Nanchang University in 2022. She is currently pursuing a Master’s degree in Computer Science and Technology at Fudan University, Shanghai, China. Her research interests include artificial intelligence, computer vision, and video object segmentation.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{TCSVT-ClickVOS/bio/JinglunLi.jpg}}]{Jinglun Li}
obtained a master's degree in Software Engineering in 2021 from Beijing University of Posts and Telecommunications. He is recently pursuing an Eng.D. in Computer Technology and Engineering at Fudan University. His current research interests include OOD detection, image segmentation, AIGC, and other areas within deep learning and machine learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{TCSVT-ClickVOS/bio/ZhaoyuChen.jpg}}]{Zhaoyu Chen}
received B.Eng. degree from Shandong University by 2020. He is currently pursuing the Ph.D. degree with the Academy for Engineering and Technology, Fudan University, Shanghai. His research interests include artificial intelligence security, computer vision, and their applications, such as adversarial examples and semantic segmentation.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{TCSVT-ClickVOS/bio/XiaoqiangLi.jpeg}}]{Xiaoqiang Li}
received the Ph.D. degree in computer science from Fudan University, Shanghai, China, in 2004. He is currently an Associate Professor of computer science with Shanghai University, China. His current research interests include image processing, pattern recognition, computer vision, and machine learning. He is currently an ACM Member, a Senior Member of the Chinese Computer Society, and a Deputy Director of the Multimedia Special Committee of the Shanghai Computer Society.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{TCSVT-ClickVOS/bio/WeiZhang.png}}]{Wei Zhang}
received the Ph.D. degree in computer science from Fudan University, China, in 2008. He was a Visiting Scholar at the UNC-Charlotte from 2016 to 2017. He is currently an Associate Professor with the School of Computer Science, Fudan University. His current research interests include deep learning, computer vision, and video object segmentation.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{TCSVT-ClickVOS/bio/WenqiangZhang.png}}]{Wenqiang Zhang}
received the Ph.D. degree in mechanical engineering from Shanghai Jiao Tong University, China, in 2004. He is currently a Professor with the School of Computer Science, Fudan University. His current research interests include computer vision and robot intelligence.
\end{IEEEbiography}

\vfill
